Are Emojis Emotional? A Study to Understand the Association between Emojis and Emotions

Given the growing ubiquity of emojis in language, there is a need for methods and resources that shed light on their meaning and communicative role. One conspicuous aspect of emojis is their use to convey affect in ways that may otherwise be non-trivial to achieve. In this paper, we seek to explore the connection between emojis and emotions by means of a new dataset consisting of human-solicited association ratings. We additionally conduct experiments to assess to what extent such associations can be inferred from existing data, such that similar associations can be predicted for a larger set of emojis. Our experiments show that this succeeds when high-quality word-level information is available.

==> tab-affect-intensity.tex <==
\begin{table}
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\makecell{Top K\\Words}} & \textbf{\makecell{Score\\Groups}} & \textbf{A} & \textbf{F} & \textbf{J} & \textbf{S} & \textbf{Avg} \\ \hline

10 & All  & 0.27	& 0.42	& 0.63	&0.47 &	0.45 \\
& 0.5-1   & -0.55   & 0.56  & 0.23    & 0.27 &  0.13 \\ \hline

25 & All  &0.34	&0.59	&0.65	&0.62 & 0.55 \\
& 0.5-1   &0.58    &0.74    &0.25    &0.43 & 0.50 \\ \hline

\textbf{100} &   All &   \textbf{0.45}  &\textbf{0.65}	&\textbf{0.70}   &\textbf{0.70}	&\textbf{0.63} \\ 
& 0.5-1 &\textbf{0.84}    &\textbf{0.86}    &\textbf{0.16}    &\textbf{0.47} & \textbf{0.58}\\ \hline

150 & All & 0.48	&0.66	&0.69	&0.68 & 0.63 \\	
& 0.5-1 & 0.86    &0.87    &0.11    &0.37 & 0.55 \\ \hline

300 & All & 0.48	    &0.66	&0.69    &0.63	& 0.62 \\
& 0.5-1 & 0.76    &0.87     &0.04    &0.41 & 0.52 \\ \hline

\end{tabular}
\caption{The Pearson correlation between gold scores and prediction anger (A), fear (F), joy (J), sadness (S), average (Avg) when using Affect Intensity lexicon in the prediction}
\label{tab:affect-intensity}
\end{table}

==> tab-depeche-mood.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{\makecell{Top K\\Words}} & \textbf{\makecell{Minimum Word\\Frequency}} & \textbf{\makecell{Score\\Groups}} & \textbf{\makecell{Afraid}} & \textbf{Amused} & \textbf{Angry} & \textbf{Annoyed}  & \textbf{Happy} & \textbf{Sad} & \textbf{Average} \\ \hline

	& 0	    & All	&   0.17	& \textbf{0.14}  & 0.19	& 0.37	 & 0.44 	& 0.57	& 0.31 \\ 
	& 	    & 0.5-1	&   -0.03	& 0.17  & 0.09	& 0.44	 & -0.05	& 0.48	& 0.18 \\ 
50	& 25	& All	&   0.22    & 0.12  & 0.20  & \textbf{0.42}   & 0.48     & 0.58	& 0.34 \\ 
	& 	    & 0.5-1	&   \textbf{0.15}    & 0.02  & 0.05  & 0.52   & \textbf{0.02}     & 0.35	& 0.19 \\ 
	& 50	& All	&   0.21	& 0.07  & 0.23	& 0.36	 & 0.45	    & 0.62	& 0.32 \\ 
	& 	    & 0.5-1	&   0.08	& 0.18  & -0.04	& 0.69	 & -0.01	& 0.37	& \textbf{0.21} \\ \hline

	& 0	    & All	&   0.32	& 0.11  & 0.20	& 0.34	 & 0.43	    & 0.67	& 0.35 \\ 
	& 	    & 0.5-1	&   -0.20	& -0.01 & 0.01	& \textbf{0.95}	 & -0.04	& \textbf{0.51}	& 0.02 \\ 
100	& 25	& All	&   \textbf{0.33}	& 0.09  & 0.29	& 0.37	 & 0.48 	& 0.68	& \textbf{0.37} \\ 
	& 	    & 0.5-1	&   -0.04	& 0.41  & -0.05	& 0.37	 & -0.09	& 0.45	& 0.18 \\ 
	& 50	& All	&   0.31	& 0.06  & 0.29	& 0.36	 & \textbf{0.49} 	& 0.69	& \textbf{0.37} \\ 
	& 	    & 0.5-1	&   -0.01	& \textbf{0.49}  & -0.26	& 0.39	 & -0.05	& 0.50	& 0.18 \\ \hline
	
	& 0	    & All	&   0.24	& 0.09  & 0.24	& 0.36	 & 0.42 	& 0.70	& 0.34 \\ 
	& 	    & 0.5-1	&   -0.13	& -0.02 & 0.04	& 0.74	 & -0.20	& 0.48	& 0.15 \\ 
150	& 25	& All	&   0.28    & 0.07  & 0.32  & 0.36   & 0.40     & 0.72	& 0.36 \\ 
	& 	    & 0.5-1	&   -0.09   & -0.10 & \textbf{0.16}  & 0.41   & -0.17    & 0.49	& 0.12 \\ 
	& 50	& All	&   0.27	& 0.05  & 0.34	& 0.36	 & 0.40	    & 0.72	& 0.36 \\ 
	& 	    & 0.5-1	&   0.07	& -0.02 & 0.10	& 0.55	 & -0.18	& 0.46	& 0.16 \\ \hline
	
	& 0	    & All	&   0.19	& 0.13  & 0.25	& 0.35	 & 0.36 	& 0.69	& 0.33 \\ 
	& 	    & 0.5-1	&   0.04	& -0.30 & 0.01	& 0.34	 & -0.13	& 0.41	& 0.06 \\ 
200	& 25	& All	&   0.27    & 0.12  & 0.31  & 0.37   & 0.35     & 0.72	& 0.36 \\ 
	& 	    & 0.5-1	&   0.11    & -0.35 & 0.06  & 0.39   & -0.17    & 0.38	& 0.07 \\ 
	& 50	& All	&   0.28	& 0.09  & \textbf{0.34}	& 0.38	 & 0.36	    & \textbf{0.73}	& 0.36 \\ 
	& 	    & 0.5-1	&   0.03	& -0.23 & 0.19	& 0.45	 & -0.17	& 0.43	& 0.12 \\ \hline


\end{tabular}
\caption{The Pearson Correlation score between human annotated emotion score and our predicted score using DepecheMood++}
\label{tab:depeche-mood}
\end{table*}

==> tab-discussion.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Source} & \textbf{\makecell{Score\\Groups}} & \textbf{Anger} & \textbf{Anticipation} & \textbf{Disgust} & \textbf{\makecell{Fear}} & \textbf{\makecell{Joy}} & \textbf{Sadness}  & \textbf{Surprise} & \textbf{Trust} & \textbf{Average} \\ \hline

EmoLex & All & 0.52	& \textcolor{red}{-0.21}	    & \textbf{0.76}	&   0.41	& 0.14	& 0.5	 & -0.33	& \textbf{0.03}	& 0.23 \\ 
& 0.5-1 & 0.57 & \textcolor{red}{-0.95} & \textcolor{red}{-0.27} & 0.03	& -0.43	& -0.77	& -0.56	& \textbf{0.34} & -0.26 \\ \hline

\makecell{Affect\\Intensity\\(Sim. Based)} & All & 0.45	& X	    & X	& \textbf{0.65}	& \textbf{0.70}	& \textbf{0.70}	 & X	& X	& 0.63 \\ 
                             & 0.5-1 & 0.84 & X     & X & \textbf{0.86}	& \textbf{0.16}	& 0.47	& X	& X & \textbf{0.58} \\ \hline
\makecell{Affect\\Intensity\\(Freq. Based)} & All & \textbf{0.62}	& X	    & X	&   0.58	& 0.65	& \textbf{0.70}	 & X	& X	& \textbf{0.64} \\ 
                             & 0.5-1 & \textbf{0.92} & X     & X & 0.77	& -0.04	& \textbf{0.49}	& X	& X & 0.54 \\ \hline
                             
\makecell{Depeche\\Mood++} & All & 0.33	& X	    & X	&   0.33	& 0.48	& 0.68	 & \textbf{0.09}	& X	& 0.38 \\ 
                             & 0.5-1 & 0.16 & X     & X & -0.04	& -0.09	& 0.45	& \textbf{0.41}	& X & 0.18 \\ \hline
\end{tabular}
}
\caption{A comparison of the Pearson Correlation scores for different methods considered in the experiments.}
\label{tab:discussion}
\end{table*}

==> tab-emo-word-count.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|}

\hline
\textbf{Emoji}    &\textbf{Emotion} & \textbf{\makecell{Cooccurring\\Words}}  \\ \hline

\includegraphics[height=\fontcharht\font`\H]{twitter-emoji-v2/1f62d.png}  Loudly crying face & Anger & \makecell{w1,w2\\w3,w4,w5} \\ \hline

\includegraphics[height=\fontcharht\font`\H]{twitter-emoji-v2/1f62d.png}  Loudly crying face & Fear & \makecell{w1,w2\\w3,w4,w5} \\ \hline

\includegraphics[height=\fontcharht\font`\H]{twitter-emoji-v2/1f62d.png}  Loudly crying face & Joy & \makecell{w1,w2\\w3,w4,w5} \\ \hline

\end{tabular}
\caption{Co-occurring Emojis and Words grouped by Emotion}
\label{tab:emo-word-count}
\end{table}

==> tab-emo-word-result.tex <==
\begin{table}
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\makecell{Top K\\Words}} & \textbf{\makecell{Score\\Groups}} & \textbf{A} & \textbf{F} & \textbf{J} & \textbf{S} & \textbf{Avg} \\ \hline

25 & All &0.42	&0.58	&0.68	&0.68	& 0.59 \\
& 0.5-1   &0.86    &0.66    &0.12    &0.49    & 0.53 \\ \hline

\textbf{100} &   All &   \textbf{0.62}  &\textbf{0.58}	&\textbf{0.65}   &\textbf{0.70}	& \textbf{0.64} \\ 
                & 0.5-1 & \textbf{0.92}  &\textbf{0.77}   &\textbf{-0.04}   &\textbf{0.49} & \textbf{0.54} \\ \hline

150 & All & 0.62	    &0.61	&0.65	&0.69 & 0.64 \\	
& 0.5-1 & 0.79    &0.67    &0.0    &0.24 & 0.42 \\ \hline

\end{tabular}
\caption{Pearson correlation between gold and prediction for anger (A), fear (F), joy (J), sadness (S), average (Avg) when using Word-Emoji Cooccurrence lexicon}
\label{tab:emo-word-result}
\end{table}

==> tab-emolex.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{\makecell{Score\\Groups}} & \textbf{Anger} & \textbf{Anticipation} & \textbf{Disgust} & \textbf{\makecell{Fear}} & \textbf{\makecell{Joy}} & \textbf{Sadness}  & \textbf{Surprise} & \textbf{Trust} & \textbf{Average} \\ \hline

All & 0.52	& -0.21	    & 0.76	&   0.41	& 0.14	& 0.5	 & -0.33	& 0.03	& 0.23 \\ 
0.5-1 & 0.57 & -0.95 & -0.27 & 0.03	& -0.43	& -0.77	& -0.56	& 0.34 & -0.26 \\ \hline
\end{tabular}
\caption{The Pearson correlation score between gold score and our predicted emotion score using EmoLex}
\label{tab:emolex}
\end{table*}

==> tab-pearson.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{0.5em} %
\renewcommand{\arraystretch}{1.5}%
\begin{tabular}{c c c c c}
 & \textbf{R1}  & \textbf{R2} & \textbf{R3} & \textbf{R4} \\ 
\textbf{R5} & \cellcolor{green!80} \textbf{0.65}  & \cellcolor{green!50}\textbf{0.54} & \cellcolor{green!50} \textbf{0.53} & \cellcolor{green!40}\textbf{0.48} \\ 
\textbf{R4} & \cellcolor{yellow!70} \textbf{0.53}  & \cellcolor{yellow!60}\textbf{0.51} & \cellcolor{yellow!60}\textbf{0.50} &  \\ 
\textbf{R3} & \cellcolor{blue!40}\textbf{0.53}  & \cellcolor{blue!15} \textbf{0.42} &  &  \\ 
\textbf{R2} & \cellcolor{orange!70} \textbf{0.57}  &  &  &  \\ 

\end{tabular}
\caption{Pairwise Pearson Correlation for 5 raters based on all 8 emotion scores for the set of 150 most popular Twitter emojis}
\label{tab:correlation}
\end{table}

==> tab-spearman.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{0.5em} %
\renewcommand{\arraystretch}{1.5}%
\begin{tabular}{c c c c c}
 & \textbf{R1}  & \textbf{R2} & \textbf{R3} & \textbf{R4} \\ 
\textbf{R5} & \cellcolor{green!80} \textbf{0.59}  & \cellcolor{green!50}\textbf{0.51} & \cellcolor{green!25} \textbf{0.52} & \cellcolor{green!15}\textbf{0.44} \\ 
\textbf{R4} & \cellcolor{yellow!70} \textbf{0.48}  & \cellcolor{yellow!30}\textbf{0.43} & \cellcolor{yellow!70}\textbf{0.48} &  \\ 
\textbf{R3} & \cellcolor{blue!40}\textbf{0.53}  & \cellcolor{blue!15} \textbf{0.40} &  &  \\ 
\textbf{R2} & \cellcolor{orange!70} \textbf{0.53}  &  &  &  \\ 


\end{tabular}
\caption{Pairwise Spearman Rank Correlation for 5 raters based on all 8 emotion scores for the set of 150 most popular Twitter emojis}
\label{tab:correlation}
\end{table}
